An Interpreter for Quantum Circuits

This paper describes an ACL2 interpreter for "netlists" describing quantum circuits. Several quantum gates are implemented, including the Hadamard gate H, which rotates vectors by 45 degrees, necessitating the use of irrational numbers, at least at the logical level. Quantum measurement presents an especially difficult challenge, because it requires precise comparisons of irrational numbers and the use of random numbers. This paper does not address computation with irrational numbers or the generation of random numbers, although future work includes the development of pseudo-random generators for ACL2.

==> eptcsdata.tex <==
\providecommand{\firstpage}{85}
\providecommand{\publicationstatus}{R. Gamboa and J. Davis (Eds.): ACL2 Workshop 2013 (ACL2 '13).\\
EPTCS 114, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.114.7}{10.4204/EPTCS.114.7}}

